A theoretical study of top-mass measurements at the LHC using NLO+PS generators of increasing accuracy

In this paper we study the theoretical uncertainties in the determination of the top-quark mass using next-to-leading-order (NLO) generators interfaced to parton showers (PS) that have different levels of accuracy. Specifically we consider three generators: one that implements NLO corrections in the production dynamics, one that includes also NLO corrections in top decay in the narrow width approximation, and one that implements NLO corrections for both production and decay including finite-width and interference effects. Since our aim is to provide an assessment of the uncertainties of purely theoretical origin, we consider simplified top-mass related observables that are broadly related to those effectively used by experiments, eventually modelling experimental resolution effects with simple smearing procedures. We estimate the differences in the value of the extracted top mass that would occur due to the use of the three different NLO generators, to the variation of scales, to the choice of parton distribution functions and to the matching procedure. Furthermore, we also consider differences due to the shower and to the modelling of non-perturbative effects by interfacing our NLO generators to both Pythia8.2 and Herwig7.1, with various settings. We find very different results depending upon the adopted shower model. While with Pythia8.2 we find moderate differences between the different NLO+PS generators, with Herwig7.1 we find very large ones. Furthermore, the differences between Pythia8.2 and Herwig7.1 generators are also remarkably large.

==> tables/MEC_POWHEG_hw7_table.tex <==
 \begin{tabular}{l|c|c|c|c|}
 \cline{2-5}
 &  \multicolumn{2}{ |c|}{ \phantom{\Big|} No smearing}
 &  \multicolumn{2}{ |c|}{15~GeV smearing} \\
 \cline{2-5}
 & \phantom{\Big|} {\tt POWHEG} & {\tt POWHEG} ${}-$ MEC
 & \phantom{\Big|} {\tt POWHEG} & {\tt POWHEG} ${}-$ MEC\\
 \cline{1-5}
 \multicolumn{1}{ |c|  }{ \phantom{\Big|}\bbfourl{}}
 & $172.475\pm   0.005$~GeV 
  &  $        -252 \pm            8 $~MeV 
 & $171.219\pm   0.002$~GeV  
  &  $        -407 \pm            2 $~MeV 
 \\ \cline{1-5}
 \multicolumn{1}{ |c|  }{ \phantom{\Big|}\ttbnlodec{}}
 & $172.444\pm   0.004$~GeV 
  &  $        -333 \pm            6 $~MeV 
 & $171.084\pm   0.001$~GeV  
  &  $        -591 \pm            2 $~MeV 
 \\ \cline{1-5}
 \multicolumn{1}{ |c|  }{ \phantom{\Big|}\hvq{}}
 & $172.794\pm   0.004$~GeV 
  &  $        -244 \pm            6 $~MeV 
 & $171.963\pm   0.001$~GeV  
  &  $        -356 \pm            2 $~MeV 
 \\ \cline{1-5}
\end{tabular}


==> tables/MEC_POWHEG_hw7_table_lept.tex <==
 \begin{tabular}{c|c|c|c|}
 \cline{2-4}
 &  \multicolumn{3}{ |c|}{$\phantom{\Big|}$  MEC ${}-$ POWHEG} \\
 \cline{2-4}
 & $\phantom{\Big|}$  \tt \bbfourl & \ttbnlodec & \hvq{}\\
 \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)\rangle $}
 & $+    55\pm
    106$~MeV 
 & $+    96\pm
     74$~MeV 
 & $+    65\pm
     58$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+\ell^-)\rangle $}
 & $+   112\pm
    127$~MeV 
 & $+   157\pm
     89$~MeV 
 & $+   177\pm
     68$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle m(\ell^+\ell^-)\rangle $}
 & $+   108\pm
    215$~MeV 
 & $+   204\pm
    147$~MeV 
 & $+   104\pm
    114$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle E(\ell^+\ell^-)\rangle $}
 & $+   220\pm
    348$~MeV 
 & $+   314\pm
    243$~MeV 
 & $+   285\pm
    188$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)+\pT(\ell^-)\rangle $}
 & $+   130\pm
    205$~MeV 
 & $+   156\pm
    141$~MeV 
 & $+   160\pm
    110$~MeV 
\\ \cline{1-4}
\end{tabular}


==> tables/allradii-lept.tex <==
\begin{tabular}{lc||c|c||c|c||}
\\ \cline{3-6}
 & & \multicolumn{4}{ |c||}{$\phantom{\Big|}$ $ \langle O(R=\%) \rangle - \langle O(R=0.5) \rangle$ [MeV]}
\\ \cline{3-6}
 & & \multicolumn{2}{ |c||}{\phantom{\Big|} \PythiaEight} & \multicolumn{2}{ |c||}{\HerwigSeven}
\\ \cline{1-6}
\multicolumn{1}{ |c|}{observable \phantom{\Big|}}  & \multicolumn{1}{ |c||}{generator}
 & $R=0.4$ & $R=0.6$
 & $R=0.4$ & $R=0.6$
\\ \cline{1-6}
\\[-1.25em]
\cline{1-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl $\phantom{\Big|}$}
 & $   -147 \pm
     71 $ 
 & $+   135 \pm
     70 $ 
 & $   -101 \pm
     70 $ 
 & $+   113 \pm
     69 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)\rangle $} & \multicolumn{1}{ |c||}{\ttbnlodec $\phantom{\Big|}$}
 & $   -138 \pm
     47 $ 
 & $+   147 \pm
     46 $ 
 & $   -112 \pm
     67 $ 
 & $+   133 \pm
     57 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq $\phantom{\Big|}$ }
 & $   -146 \pm
     46 $ 
 & $+   149 \pm
     45 $ 
 & $   -118 \pm
     46 $ 
 & $+   118 \pm
     45 $ 
\\ \cline{2-6}
\cline{1-6}
\\[-1.25em]
\cline{1-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl $\phantom{\Big|}$}
 & $    -54 \pm
     84 $ 
 & $+    20 \pm
     83 $ 
 & $    -14 \pm
     84 $ 
 & $+     6 \pm
     82 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c||}{\ttbnlodec $\phantom{\Big|}$}
 & $    -32 \pm
     57 $ 
 & $+    19 \pm
     55 $ 
 & $     -6 \pm
     73 $ 
 & $+    20 \pm
     64 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq $\phantom{\Big|}$ }
 & $    -47 \pm
     55 $ 
 & $+    23 \pm
     54 $ 
 & $    -28 \pm
     54 $ 
 & $+     9 \pm
     53 $ 
\\ \cline{2-6}
\cline{1-6}
\\[-1.25em]
\cline{1-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl $\phantom{\Big|}$}
 & $   -418 \pm
    142 $ 
 & $+   428 \pm
    140 $ 
 & $   -345 \pm
    141 $ 
 & $+   371 \pm
    139 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{$\langle m(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c||}{\ttbnlodec $\phantom{\Big|}$}
 & $   -418 \pm
     92 $ 
 & $+   450 \pm
     91 $ 
 & $   -352 \pm
    103 $ 
 & $+   382 \pm
     97 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq $\phantom{\Big|}$ }
 & $   -417 \pm
     91 $ 
 & $+   445 \pm
     89 $ 
 & $   -362 \pm
     90 $ 
 & $+   398 \pm
     89 $ 
\\ \cline{2-6}
\cline{1-6}
\\[-1.25em]
\cline{1-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl $\phantom{\Big|}$}
 & $   -414 \pm
    232 $ 
 & $+   333 \pm
    228 $ 
 & $   -313 \pm
    230 $ 
 & $+   295 \pm
    227 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{$\langle E(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c||}{\ttbnlodec $\phantom{\Big|}$}
 & $   -398 \pm
    154 $ 
 & $+   387 \pm
    150 $ 
 & $   -312 \pm
    169 $ 
 & $+   306 \pm
    159 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq $\phantom{\Big|}$ }
 & $   -399 \pm
    151 $ 
 & $+   388 \pm
    147 $ 
 & $   -333 \pm
    149 $ 
 & $+   342 \pm
    146 $ 
\\ \cline{2-6}
\cline{1-6}
\\[-1.25em]
\cline{1-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl $\phantom{\Big|}$}
 & $   -291 \pm
    136 $ 
 & $+   274 \pm
    134 $ 
 & $   -212 \pm
    135 $ 
 & $+   227 \pm
    133 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)+\pT(\ell^-)\rangle $} & \multicolumn{1}{ |c||}{\ttbnlodec $\phantom{\Big|}$}
 & $   -281 \pm
     90 $ 
 & $+   289 \pm
     88 $ 
 & $   -215 \pm
    110 $ 
 & $+   246 \pm
     99 $ 
\\ \cline{2-6}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq $\phantom{\Big|}$ }
 & $   -284 \pm
     88 $ 
 & $+   287 \pm
     86 $ 
 & $   -230 \pm
     87 $ 
 & $+   245 \pm
     85 $ 
\\ \cline{2-6}
\cline{1-6}
\\[-1.25em]
\cline{1-6}
\end{tabular}


==> tables/allradii-showerOnly-lept.tex <==
\begin{tabular}{lc||c|c||c|c||c|c||c|c||}
\\ \cline{3-10}
 & & \multicolumn{8}{ |c||}{$\phantom{\Big|}$ $ \langle O(R=\%) \rangle - \langle O(R=0.5) \rangle$ [MeV]}
\\ \cline{3-10}
 & & \multicolumn{2}{ |c||}{\phantom{\Big|} \PythiaEight{} full} & \multicolumn{2}{ |c||}{\HerwigSeven{} full}& \multicolumn{2}{ |c||}{\phantom{\Big|} \PythiaEight{} NLO+PS} & \multicolumn{2}{ |c||}{\HerwigSeven{} NLO+PS}
\\ \cline{1-10}
\multicolumn{1}{ |c|}{\phantom{\Big|}observable \phantom{\Big|}}  & \multicolumn{1}{ |c||}{gen}
 & $R=0.4$ & $R=0.6$
 & $R=0.4$ & $R=0.6$
 & $R=0.4$ & $R=0.6$
 & $R=0.4$ & $R=0.6$
\\ \cline{1-10}
\\[-1.25em]
\cline{1-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl\!\!\!\! $\phantom{\Big|}$}
 & $   -147 \pm
     71 $ 
 & $+   135 \pm
     70 $ 
 & $   -101 \pm
     70 $ 
 & $+   113 \pm
     69 $ 
 & $    -94 \pm
     72 $ 
 & $+    99 \pm
     71 $ 
 & $    -65 \pm
     71 $ 
 & $+    74 \pm
     70 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{\!\!\!$\langle \pT(\ell^+)\rangle $\!\!\!} & \multicolumn{1}{ |c||}{\ttbnlodec $\!\!\!\phantom{\Big|}$}
 & $   -138 \pm
     47 $ 
 & $+   147 \pm
     46 $ 
 & $   -112 \pm
     67 $ 
 & $+   133 \pm
     57 $ 
 & $    -92 \pm
     49 $ 
 & $+    98 \pm
     48 $ 
 & $    -70 \pm
     49 $ 
 & $+    75 \pm
     48 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq \!\!\!$\phantom{\Big|}$ }
 & $   -146 \pm
     46 $ 
 & $+   149 \pm
     45 $ 
 & $   -118 \pm
     46 $ 
 & $+   118 \pm
     45 $ 
 & $    -92 \pm
     47 $ 
 & $+    86 \pm
     46 $ 
 & $    -78 \pm
     46 $ 
 & $+    83 \pm
     45 $ 
\\ \cline{2-10}
\cline{1-10}
\\[-1.25em]
\cline{1-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl\!\!\!\! $\phantom{\Big|}$}
 & $    -54 \pm
     84 $ 
 & $+    20 \pm
     83 $ 
 & $    -14 \pm
     84 $ 
 & $+     6 \pm
     82 $ 
 & $    -21 \pm
     86 $ 
 & $+     1 \pm
     84 $ 
 & $     -2 \pm
     84 $ 
 & $     -7 \pm
     83 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{\!\!\!$\langle \pT(\ell^+\ell^-)\rangle $\!\!\!} & \multicolumn{1}{ |c||}{\ttbnlodec $\!\!\!\phantom{\Big|}$}
 & $    -32 \pm
     57 $ 
 & $+    19 \pm
     55 $ 
 & $     -6 \pm
     73 $ 
 & $+    20 \pm
     64 $ 
 & $    -19 \pm
     59 $ 
 & $     -2 \pm
     58 $ 
 & $+     9 \pm
     60 $ 
 & $    -11 \pm
     59 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq \!\!\!$\phantom{\Big|}$ }
 & $    -47 \pm
     55 $ 
 & $+    23 \pm
     54 $ 
 & $    -28 \pm
     54 $ 
 & $+     9 \pm
     53 $ 
 & $    -22 \pm
     56 $ 
 & $     -2 \pm
     55 $ 
 & $     -7 \pm
     55 $ 
 & $     -9 \pm
     54 $ 
\\ \cline{2-10}
\cline{1-10}
\\[-1.25em]
\cline{1-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl\!\!\!\! $\phantom{\Big|}$}
 & $   -418 \pm
    142 $ 
 & $+   428 \pm
    140 $ 
 & $   -345 \pm
    141 $ 
 & $+   371 \pm
    139 $ 
 & $   -303 \pm
    143 $ 
 & $+   327 \pm
    142 $ 
 & $   -240 \pm
    142 $ 
 & $+   280 \pm
    141 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{\!\!\!$\langle m(\ell^+\ell^-)\rangle $\!\!\!} & \multicolumn{1}{ |c||}{\ttbnlodec $\!\!\!\phantom{\Big|}$}
 & $   -418 \pm
     92 $ 
 & $+   450 \pm
     91 $ 
 & $   -352 \pm
    103 $ 
 & $+   382 \pm
     97 $ 
 & $   -304 \pm
     99 $ 
 & $+   339 \pm
     97 $ 
 & $   -259 \pm
    100 $ 
 & $+   288 \pm
     99 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq \!\!\!$\phantom{\Big|}$ }
 & $   -417 \pm
     91 $ 
 & $+   445 \pm
     89 $ 
 & $   -362 \pm
     90 $ 
 & $+   398 \pm
     89 $ 
 & $   -302 \pm
     93 $ 
 & $+   318 \pm
     91 $ 
 & $   -261 \pm
     91 $ 
 & $+   296 \pm
     90 $ 
\\ \cline{2-10}
\cline{1-10}
\\[-1.25em]
\cline{1-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl\!\!\!\! $\phantom{\Big|}$}
 & $   -414 \pm
    232 $ 
 & $+   333 \pm
    228 $ 
 & $   -313 \pm
    230 $ 
 & $+   295 \pm
    227 $ 
 & $   -292 \pm
    235 $ 
 & $+   255 \pm
    232 $ 
 & $   -188 \pm
    232 $ 
 & $+   212 \pm
    230 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{\!\!\!$\langle E(\ell^+\ell^-)\rangle $\!\!\!} & \multicolumn{1}{ |c||}{\ttbnlodec $\!\!\!\phantom{\Big|}$}
 & $   -398 \pm
    154 $ 
 & $+   387 \pm
    150 $ 
 & $   -312 \pm
    169 $ 
 & $+   306 \pm
    159 $ 
 & $   -284 \pm
    160 $ 
 & $+   283 \pm
    157 $ 
 & $   -204 \pm
    161 $ 
 & $+   210 \pm
    159 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq \!\!\!$\phantom{\Big|}$ }
 & $   -399 \pm
    151 $ 
 & $+   388 \pm
    147 $ 
 & $   -333 \pm
    149 $ 
 & $+   342 \pm
    146 $ 
 & $   -280 \pm
    154 $ 
 & $+   261 \pm
    151 $ 
 & $   -225 \pm
    150 $ 
 & $+   236 \pm
    148 $ 
\\ \cline{2-10}
\cline{1-10}
\\[-1.25em]
\cline{1-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\bbfourl\!\!\!\! $\phantom{\Big|}$}
 & $   -291 \pm
    136 $ 
 & $+   274 \pm
    134 $ 
 & $   -212 \pm
    135 $ 
 & $+   227 \pm
    133 $ 
 & $   -189 \pm
    138 $ 
 & $+   185 \pm
    136 $ 
 & $   -138 \pm
    136 $ 
 & $+   155 \pm
    135 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{\!\!\!$\langle \pT(\ell^+)+\pT(\ell^-)\rangle $\!\!\!} & \multicolumn{1}{ |c||}{\ttbnlodec $\!\!\!\phantom{\Big|}$}
 & $   -281 \pm
     90 $ 
 & $+   289 \pm
     88 $ 
 & $   -215 \pm
    110 $ 
 & $+   246 \pm
     99 $ 
 & $   -189 \pm
     92 $ 
 & $+   188 \pm
     91 $ 
 & $   -138 \pm
     93 $ 
 & $+   155 \pm
     92 $ 
\\ \cline{2-10}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c||}{\hvq \!\!\!$\phantom{\Big|}$ }
 & $   -284 \pm
     88 $ 
 & $+   287 \pm
     86 $ 
 & $   -230 \pm
     87 $ 
 & $+   245 \pm
     85 $ 
 & $   -184 \pm
     90 $ 
 & $+   175 \pm
     88 $ 
 & $   -153 \pm
     88 $ 
 & $+   166 \pm
     86 $ 
\\ \cline{2-10}
\cline{1-10}
\\[-1.25em]
\cline{1-10}
\end{tabular}


==> tables/cmp_bb4l_showerOnly_Ebj.tex <==
 \begin{tabular}{l|c|c|}
 \cline{2-3}
 & $\phantom{\Big|}$ PS only & full \\ 
 \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \ttbnlodec{} ${}-$ \bbfourl{} }
 & $+   411\pm    103 $~MeV
 & $+   161\pm    102 $~MeV
\\ \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \hvq{} ${}-$ \bbfourl{} }
 & $   -257\pm    104 $~MeV
 & $   -456\pm    103 $~MeV
\\ \cline{1-3}
\end{tabular}


==> tables/cmp_generators_shower_lept.tex <==
 \begin{tabular}{c|c|c|c|}
 \cline{2-4}
 &  \multicolumn{3}{ |c|}{$\phantom{\Big|}$  \PythiaEightPtwo{} ${}-$ \HerwigSevenPone{}} \\
 \cline{2-4}
 & $\phantom{\Big|}$  \tt \bbfourl & \ttbnlodec & \hvq{}\\
 \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)\rangle $}
 & $+   554\pm
     78$~MeV 
 & $+   605\pm
     57$~MeV 
 & $+   340\pm
     45$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+\ell^-)\rangle $}
 & $+  1099\pm
     93$~MeV 
 & $+  1027\pm
     65$~MeV 
 & $+   636\pm
     54$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle m(\ell^+\ell^-)\rangle $}
 & $+   189\pm
    156$~MeV 
 & $+   736\pm
     97$~MeV 
 & $+   144\pm
     90$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle E(\ell^+\ell^-)\rangle $}
 & $+  1266\pm
    256$~MeV 
 & $+  1690\pm
    160$~MeV 
 & $+   684\pm
    148$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)+\pT(\ell^-)\rangle $}
 & $+  1052\pm
    150$~MeV 
 & $+  1143\pm
     99$~MeV 
 & $+   629\pm
     86$~MeV 
\\ \cline{1-4}
\end{tabular}


==> tables/cmp_shower_Ebj.tex <==
 \newcommand\myspace{\hspace{-2mm}}
 \begin{tabular}{l|c|c|c|}
 \cline{2-4}
 & \multicolumn{3}{|c|}{$\phantom{\Big|}$ \PythiaEightPtwo{} ${}-$ \HerwigSevenPone{}   } \\
 \cline{2-4}
 & \multicolumn{1}{|c|}{$\phantom{\Big|}$ $R=0.4$}  & \multicolumn{1}{|c|}{$R=0.5$}  & \multicolumn{1}{|c|}{$R=0.6$} \\
 \cline{1-4}
\multicolumn{1}{ |c|}{  \myspace $\phantom{\Big|}$ \bbfourl{}}
 & $   1631\pm    122 $~MeV
 & $   2150\pm    114 $~MeV
 & $   2356\pm    113 $~MeV
\\ \cline{1-4}
\multicolumn{1}{ |c|}{  \myspace $\phantom{\Big|}$ \ttbnlodec{}}
 & $   2039\pm     91 $~MeV
 & $   2332\pm     88 $~MeV
 & $   2437\pm     87 $~MeV
\\ \cline{1-4}
\multicolumn{1}{ |c|}{  \myspace $\phantom{\Big|}$ \hvq{}}
 & $    762\pm     93 $~MeV
 & $   1028\pm     89 $~MeV
 & $   1188\pm     86 $~MeV
\\ \cline{1-4}
\end{tabular}


==> tables/extracted_mass_table_lept.tex <==
 \begin{tabular}{lc|c|c|c|c|c|c|}
 \cline{3-8}
 & & \phantom{\Big|} \!\!\!$\%$ ${}-$ \bbfourl{}  & $(\muF, \muR)$ & PDF & $\as$
 & stat & {\HerwigSevenPlot} ${}-$ {\PythiaEightPlot} \\ 
 \cline{3-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} &  \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    407}^{+
    447} $
& ${}_{-    670}^{+
    670} $
& $\pm      0$   
& $\pm    362$   
& $+  2840$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $   -781$   
& ${}_{-    432}^{+
    442} $
& ${}_{-    670}^{+
    670} $
& $\pm    781$   
& $\pm    308$   
& $+  3129$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $   -440$   
& ${}_{-    426}^{+
    445} $
& ${}_{-    670}^{+
    670} $
& $\pm    440$   
& $\pm    306$   
& $+  1757$   
\\ \cline{2-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} &  \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-   2484}^{+
   1552} $
& ${}_{-    334}^{+
    334} $
& $\pm      0$   
& $\pm    293$   
& $+  3828$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $+   348$   
& ${}_{-   1880}^{+
   1264} $
& ${}_{-    334}^{+
    334} $
& $\pm    348$   
& $\pm    249$   
& $+  3594$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $+  1951$   
& ${}_{-   1933}^{+
   1285} $
& ${}_{-    334}^{+
    334} $
& $\pm   1951$   
& $\pm    247$   
& $+  2224$   
\\ \cline{2-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} &  \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    707}^{+
   1031} $
& ${}_{-   1193}^{+
   1193} $
& $\pm      0$   
& $\pm    425$   
& $+   568$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{$\langle m(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $   -384$   
& ${}_{-    739}^{+
    784} $
& ${}_{-   1193}^{+
   1193} $
& $\pm    384$   
& $\pm    358$   
& $+  2226$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $  -1555$   
& ${}_{-    746}^{+
    801} $
& ${}_{-   1193}^{+
   1193} $
& $\pm   1555$   
& $\pm    357$   
& $+   435$   
\\ \cline{2-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} &  \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    615}^{+
    692} $
& ${}_{-   1920}^{+
   1920} $
& $\pm      0$   
& $\pm    414$   
& $+  2271$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{$\langle E(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $   -362$   
& ${}_{-    806}^{+
    780} $
& ${}_{-   1920}^{+
   1920} $
& $\pm    362$   
& $\pm    350$   
& $+  3038$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $    -10$   
& ${}_{-    793}^{+
    768} $
& ${}_{-   1920}^{+
   1920} $
& $\pm     10$   
& $\pm    348$   
& $+  1230$   
\\ \cline{2-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} &  \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    425}^{+
    473} $
& ${}_{-    666}^{+
    666} $
& $\pm      0$   
& $\pm    347$   
& $+  2678$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)+\pT(\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $   -709$   
& ${}_{-    424}^{+
    448} $
& ${}_{-    666}^{+
    666} $
& $\pm    709$   
& $\pm    293$   
& $+  2939$   
\\ \cline{2-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $   -267$   
& ${}_{-    419}^{+
    454} $
& ${}_{-    666}^{+
    666} $
& $\pm    267$   
& $\pm    292$   
& $+  1618$   
\\ \cline{2-8}
\cline{1-8}
\end{tabular}


==> tables/fit_func_table.tex <==
{\renewcommand{\arraystretch}{1.25}%
\begin{table*}[htb]
\centering
\resizebox{\textwidth}{!}{
 \begin{tabular}{lc||c|c|c|c|c|c||c|c|c|c|c|c||}
 \cline{3-14}
 \\[-1.25em]
 \cline{3-14}
 &   & \multicolumn{12}{ |c||}{ $ O = O_c + B(m_t -m_{t,c})$, $O=\mwbj^{\rm max}$~[GeV]} \\
 \cline{3-14}
 &   & \multicolumn{6}{ |c||}{\PythiaEight} & \multicolumn{6}{ |c||}{\HerwigSeven}  \\
 \cline{3-14}
 \\[-1.25em]
 \cline{3-14}
 &   & $O_c$ (central) & $B$ (central) & $O_c$(lower) &  $B$ (lower) & $O_c$ (upper) & $B$ (upper)
 & $O_c$ (central) & $B$ (central) & $O_c$ (lower) & $B$ (lower) & $O_c$ (upper) & $B$ (upper) \\
\cline{1-14}
\\[-1.25em]
\cline{1-14}
 \multicolumn{1}{ ||c  }{\multirow{1}{*}{No} } &   
 \multicolumn{1}{ |c|| }{\bbllll}
&172.817& 1.0059&172.787& 1.0065&172.844& 1.0067&172.724& 1.0004&172.655& 0.9995&172.797& 1.0028\\
\cline{2-14}
 \multicolumn{1}{ ||c  }{\multirow{1}{*}{smearing} } &   
 \multicolumn{1}{ |c|| }{\ttbnlodec}
&172.823& 0.9995&172.804& 0.9995&172.835& 0.9996&172.778& 1.0027&172.719& 1.0026&172.835& 1.0026\\
\cline{2-14}
 \multicolumn{1}{ ||c  }{\multirow{1}{*}{} } &   
 \multicolumn{1}{ |c|| }{\hvq}
&172.808& 1.0022&172.794& 1.0027&172.812& 1.0022&173.036& 0.9975&173.025& 0.9972&173.042& 0.9976\\
\cline{2-14}
 \cline{1-14}
 \\[-1.25em]
 \cline{1-14}
 \multicolumn{1}{ ||c  }{\multirow{1}{*}{15 GeV} } &   
 \multicolumn{1}{ |c|| }{\bbllll}
&172.727& 0.9551&172.643& 0.9539&172.830& 0.9573&171.644& 0.9284&171.497& 0.9271&171.818& 0.9309\\
\cline{2-14}
 \multicolumn{1}{ ||c  }{\multirow{1}{*}{smearing} } &   
 \multicolumn{1}{ |c|| }{\ttbnlodec}
&172.871& 0.9568&172.809& 0.9568&172.929& 0.9568&171.691& 0.9278&171.559& 0.9278&171.819& 0.9278\\
\cline{2-14}
 \multicolumn{1}{ ||c  }{\multirow{1}{*}{} } &   
 \multicolumn{1}{ |c|| }{\hvq}
&172.570& 0.9491&172.544& 0.9490&172.582& 0.9491&172.325& 0.9343&172.294& 0.9338&172.342& 0.9343\\
\cline{2-14}
 \cline{1-14}
 \\[-1.25em]
 \cline{1-14}
\end{tabular}}
\caption{Fitted coefficients of the function $O = O_c + B(m_t -m_{t,c})$, being $O$ the peak
of the \mwbj{} distribution, $m_t$ the input mass and $m_{t,c}=172.5$~GeV, for the central,
lower and upper predictions.}
\label{tab:mass_extraction-fit_func}
\end{table*}}


==> tables/hw7_truncated_shower_table_Ebj.tex <==
 \begin{tabular}{l|c|c|}
 \cline{2-3}
 & $\phantom{\Big|}$ TS & TS ${}-$ default  \\ 
 \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \bbfourl{}}
 & $ 68.963\pm  0.083 $~GeV
 & $    -87\pm    116 $~MeV
\\ \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \ttbnlodec{}}
 & $ 69.000\pm  0.062 $~GeV
 & $    -29\pm     87 $~MeV
\\ \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \hvq{}}
 & $ 70.027\pm  0.061 $~GeV
 & $+   311\pm     87 $~MeV
\\ \cline{1-3}
\end{tabular}


==> tables/hw7_truncated_shower_table_lept.tex <==
 \begin{tabular}{c|c|c|c|}
 \cline{2-4}
 &  \multicolumn{3}{ |c|}{$\phantom{\Big|}$ TS ${}-$ default } \\
 \cline{2-4}
 & $\phantom{\Big|}$  \tt \bbfourl & \ttbnlodec & \hvq\\
 \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)\rangle $}
 & $+     7\pm
     74$~MeV 
 & $      0\pm
     58$~MeV 
 & $+    50\pm
     45$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+\ell^-)\rangle $}
 & $+    62\pm
     88$~MeV 
 & $+    46\pm
     66$~MeV 
 & $+   103\pm
     53$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle m(\ell^+\ell^-)\rangle $}
 & $   -277\pm
    148$~MeV 
 & $   -185\pm
    100$~MeV 
 & $    -83\pm
     89$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle E(\ell^+\ell^-)\rangle $}
 & $   -282\pm
    242$~MeV 
 & $   -195\pm
    163$~MeV 
 & $    -23\pm
    147$~MeV 
\\ \cline{1-4}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)+\pT(\ell^-)\rangle $}
 & $+    22\pm
    142$~MeV 
 & $     -3\pm
    101$~MeV 
 & $+   100\pm
     86$~MeV 
\\ \cline{1-4}
\end{tabular}


==> tables/matching_variations_hw7_table_lept.tex <==
 \begin{tabular}{c|c|c|}
 \cline{2-3}
 &  \multicolumn{2}{ |c|}{$\phantom{\Big|}$  {\tt ShowerVeto} ${}-$ {\tt FSV}} \\
 \cline{2-3}
 & $\phantom{\Big|}$  \tt \bbfourl & \ttbnlodec \\
 \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)\rangle $}
 & $    -86\pm
    109$~MeV 
 & $   -129\pm
     81$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+\ell^-)\rangle $}
 & $   -134\pm
    130$~MeV 
 & $   -143\pm
     94$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle m(\ell^+\ell^-)\rangle $}
 & $   -168\pm
    219$~MeV 
 & $   -209\pm
    148$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle E(\ell^+\ell^-)\rangle $}
 & $   -303\pm
    355$~MeV 
 & $   -356\pm
    245$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)+\pT(\ell^-)\rangle $}
 & $   -196\pm
    208$~MeV 
 & $   -202\pm
    147$~MeV 
\\ \cline{1-3}
\end{tabular}


==> tables/matching_variations_table_Ebj.tex <==
 \begin{tabular}{l|c|c|}
 \cline{2-3}
 & $\phantom{\Big|}$ {\tt SR}  & {\tt SR} ${}-$ {\tt FSR}\\ 
 \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \bbfourl{}}
 & $ 71.179\pm  0.082 $~GeV
 & $    -21\pm    115 $~MeV
\\ \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \ttbnlodec{}}
 & $ 71.392\pm  0.063 $~GeV
 & $+    30\pm     88 $~MeV
\\ \cline{1-3}
\end{tabular}


==> tables/matching_variations_table_hw7_Ebj.tex <==
 \begin{tabular}{l|c|c|}
 \cline{2-3}
 & $\phantom{\Big|}$ {\tt FSV} & {\tt FSV} - {\tt SV}  \\ 
 \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \bbfourl{}}
 & $ 69.190\pm  0.082$~GeV
 & $+   140\pm    115 $~MeV
\\ \cline{1-3}
\multicolumn{1}{ |c|}{ $\phantom{\Big|}$ \ttbnlodec{}}
 & $ 69.177\pm  0.063$~GeV
 & $+   148\pm     88 $~MeV
\\ \cline{1-3}
\end{tabular}


==> tables/matching_variations_table_lept.tex <==
 \begin{tabular}{c|c|c|}
 \cline{2-3}
 &  \multicolumn{2}{ |c|}{ $\phantom{\Big|}$ {\tt ScaleResonance} ${}-$ {\tt FSREmission}} \\
 \cline{2-3}
 & $\phantom{\Big|}$  \bbfourl &  \ttbnlodec\\
 \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)\rangle $}
 & $+     4\pm
     74$~MeV 
 & $+     1\pm
     47$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+\ell^-)\rangle $}
 & $     -2\pm
     89$~MeV 
 & $+     1\pm
     57$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle m(\ell^+\ell^-)\rangle $}
 & $+    37\pm
    149$~MeV 
 & $+    10\pm
     94$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle E(\ell^+\ell^-)\rangle $}
 & $+    18\pm
    243$~MeV 
 & $    -25\pm
    154$~MeV 
\\ \cline{1-3}
\multicolumn{1}{ |c|}{$\phantom{\Big|}$ $\langle \pT(\ell^+)+\pT(\ell^-)\rangle $}
 & $+    13\pm
    143$~MeV 
 & $+    17\pm
     89$~MeV 
\\ \cline{1-3}
\end{tabular}


==> tables/recoil_hw7.tex <==
 \begin{tabular}{|c||c||c|c|c|c|c|}
\cline{1-7}
\multicolumn{7}{|c|}{ \phantom{\Big|} \hvq{}, PS only } \\
\cline{1-7}
\phantom{\Big|} observable
& \PythiaEightPlot{}
& \HerwigSevenPlot{}+RecOpt:0
& \HerwigSevenPlot{}+RecOpt:1
& \HerwigSevenPlot{}+RecOpt:2
& \HerwigSevenPlot{}+RecOpt:3
& \HerwigSevenPlot{}+RecOpt:4
\\ \cline{1-7}
$\phantom{\Big|} \mwbjmax$ no smearing                                 [GeV]
& $172.498\pm  0.001$
& $172.498\pm  0.001$
& $172.497\pm  0.001$
& $172.498\pm  0.001$
& $172.500\pm  0.001$
& $172.499\pm  0.001$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{+     0\pm      2}$
& $\color{red}{     -1\pm      2}$
& $\color{red}{+     0\pm      2}$
& $\color{red}{+     2\pm      2}$
& $\color{red}{+     1\pm      2}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{     -1\pm      2}$
& $\color{blue}{+     0\pm      2}$
& $\color{blue}{+     2\pm      2}$
& $\color{blue}{+     1\pm      2}$
\\ \cline{1-7}
$\phantom{\Big|} \mwbjmax$ smearing                                    [GeV]
& $171.315\pm  0.001$
& $171.202\pm  0.001$
& $171.226\pm  0.001$
& $171.191\pm  0.001$
& $171.201\pm  0.001$
& $171.210\pm  0.001$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -113\pm      2}$
& $\color{red}{    -89\pm      2}$
& $\color{red}{   -124\pm      2}$
& $\color{red}{   -114\pm      2}$
& $\color{red}{   -105\pm      2}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{+    24\pm      2}$
& $\color{blue}{    -11\pm      2}$
& $\color{blue}{     -1\pm      2}$
& $\color{blue}{+     8\pm      2}$
\\ \cline{1-7}
$\phantom{\Big|} \Ebjmax$                                              [GeV]
& $ 69.357\pm  0.063$
& $ 68.650\pm  0.063$
& $ 68.726\pm  0.061$
& $ 68.685\pm  0.063$
& $ 68.710\pm  0.063$
& $ 68.653\pm  0.062$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -707\pm     90}$
& $\color{red}{   -631\pm     88}$
& $\color{red}{   -672\pm     90}$
& $\color{red}{   -647\pm     89}$
& $\color{red}{   -704\pm     89}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{+    76\pm     88}$
& $\color{blue}{+    35\pm     90}$
& $\color{blue}{+    60\pm     89}$
& $\color{blue}{+     3\pm     89}$
\\ \cline{1-7}
$\phantom{\Big|} \langle \pT(\ell^+)\rangle $                          [GeV]
& $ 56.682\pm  0.033$
& $ 56.306\pm  0.032$
& $ 55.997\pm  0.032$
& $ 56.428\pm  0.032$
& $ 56.327\pm  0.032$
& $ 56.270\pm  0.032$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -376\pm     46}$
& $\color{red}{   -685\pm     46}$
& $\color{red}{   -254\pm     46}$
& $\color{red}{   -355\pm     46}$
& $\color{red}{   -412\pm     46}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{   -309\pm     45}$
& $\color{blue}{+   122\pm     46}$
& $\color{blue}{+    21\pm     46}$
& $\color{blue}{    -36\pm     46}$
\\ \cline{1-7}
$\phantom{\Big|} \langle \pT(\ell^+\ell^-)\rangle $                    [GeV]
& $ 69.162\pm  0.039$
& $ 68.500\pm  0.038$
& $ 68.667\pm  0.038$
& $ 68.476\pm  0.038$
& $ 68.509\pm  0.038$
& $ 68.451\pm  0.038$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -662\pm     55}$
& $\color{red}{   -494\pm     55}$
& $\color{red}{   -685\pm     55}$
& $\color{red}{   -653\pm     55}$
& $\color{red}{   -710\pm     55}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{+   167\pm     54}$
& $\color{blue}{    -24\pm     54}$
& $\color{blue}{+     9\pm     54}$
& $\color{blue}{    -49\pm     54}$
\\ \cline{1-7}
$\phantom{\Big|} \langle m(\ell^+\ell^-)\rangle $                      [GeV]
& $109.067\pm  0.065$
& $108.884\pm  0.064$
& $107.537\pm  0.063$
& $109.555\pm  0.064$
& $108.899\pm  0.064$
& $108.829\pm  0.064$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -182\pm     91}$
& $\color{red}{  -1529\pm     91}$
& $\color{red}{+   489\pm     92}$
& $\color{red}{   -168\pm     91}$
& $\color{red}{   -237\pm     91}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{  -1347\pm     90}$
& $\color{blue}{+   671\pm     91}$
& $\color{blue}{+    14\pm     90}$
& $\color{blue}{    -55\pm     90}$
\\ \cline{1-7}
$\phantom{\Big|} \langle E(\ell^+\ell^-)\rangle $                      [GeV]
& $186.699\pm  0.107$
& $185.980\pm  0.105$
& $184.862\pm  0.105$
& $186.777\pm  0.106$
& $185.976\pm  0.105$
& $185.810\pm  0.105$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -719\pm    150}$
& $\color{red}{  -1838\pm    150}$
& $\color{red}{+    77\pm    151}$
& $\color{red}{   -723\pm    150}$
& $\color{red}{   -889\pm    150}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{  -1118\pm    148}$
& $\color{blue}{+   797\pm    150}$
& $\color{blue}{     -4\pm    149}$
& $\color{blue}{   -170\pm    149}$
\\ \cline{1-7}
$\phantom{\Big|} \langle \pT(\ell^+)+\pT(\ell^-)\rangle $              [GeV]
& $113.303\pm  0.063$
& $112.613\pm  0.061$
& $112.180\pm  0.061$
& $112.790\pm  0.062$
& $112.640\pm  0.061$
& $112.541\pm  0.061$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{red}{\PythiaEightPlot{} } [MeV]
& --
& $\color{red}{   -690\pm     88}$
& $\color{red}{  -1123\pm     88}$
& $\color{red}{   -513\pm     88}$
& $\color{red}{   -663\pm     88}$
& $\color{red}{   -762\pm     88}$
\\ \cline{2-7}
$\phantom{\Big|} \% - $\textcolor{blue}{\HerwigSevenPlot{} def} [MeV]
& --  & $+0 \pm 0$ 
& $\color{blue}{   -433\pm     87}$
& $\color{blue}{+   177\pm     87}$
& $\color{blue}{+    27\pm     87}$
& $\color{blue}{    -72\pm     87}$
\\ \cline{1-7}
 \end{tabular}


==> tables/showerOnly-lept.tex <==
\begin{tabular}{lc|c|c|}
\\ \cline{3-4}
 & & \multicolumn{2}{ |c|}{$\phantom{\Big|}$ PY8 -HW7}
\\ \cline{1-4}
 \multicolumn{1}{ |c|}{observable} & \multicolumn{1}{ |c|}{gen} & \multicolumn{1}{ |c|}{Full} & \multicolumn{1}{ |c|}{PS only}
\\ \cline{1-4}
\\[-1.25em]
\cline{1-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
 & $+   549 \pm
     70 $ 
 & $+   563 \pm
     71 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
 & $+   605 \pm
     57 $ 
 & $+   609 \pm
     48 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
 & $+   340 \pm
     45 $ 
 & $+   376 \pm
     46 $ 
\\ \cline{2-4}
\cline{1-4}
\\[-1.25em]
\cline{1-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
 & $+  1094 \pm
     83 $ 
 & $+  1092 \pm
     84 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
 & $+  1027 \pm
     65 $ 
 & $+  1020 \pm
     59 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
 & $+   636 \pm
     54 $ 
 & $+   662 \pm
     55 $ 
\\ \cline{2-4}
\cline{1-4}
\\[-1.25em]
\cline{1-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
 & $+   188 \pm
    140 $ 
 & $+   286 \pm
    142 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{$\langle m(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
 & $+   736 \pm
     97 $ 
 & $+   814 \pm
     98 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
 & $+   144 \pm
     90 $ 
 & $+   182 \pm
     91 $ 
\\ \cline{2-4}
\cline{1-4}
\\[-1.25em]
\cline{1-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
 & $+  1263 \pm
    229 $ 
 & $+  1342 \pm
    232 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{$\langle E(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
 & $+  1690 \pm
    160 $ 
 & $+  1712 \pm
    159 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
 & $+   684 \pm
    148 $ 
 & $+   719 \pm
    150 $ 
\\ \cline{2-4}
\cline{1-4}
\\[-1.25em]
\cline{1-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
 & $+  1041 \pm
    134 $ 
 & $+  1091 \pm
    136 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)+\pT(\ell^-)\rangle $} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
 & $+  1143 \pm
     99 $ 
 & $+  1173 \pm
     92 $ 
\\ \cline{2-4}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
 & $+   629 \pm
     86 $ 
 & $+   690 \pm
     88 $ 
\\ \cline{2-4}
\cline{1-4}
\\[-1.25em]
\cline{1-4}
\end{tabular}


==> tables/th_error_table_lept_old.tex <==
 \begin{tabular}{lcc|c|c|c|c|c|}
\cline{1-8}
\multicolumn{1}{ |c|}{Obs $\phantom{\Big|}$} & \multicolumn{1}{ |c|}{B} & \multicolumn{1}{ |c|}{generator}
 & $\%$ ${}-$ \bbfourl & $(\muF, \muR )$ & PDF & $\as$  & stat \\
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-     85}^{+     77} $
& ${}_{-    130}^{+    130} $
& $\pm     26$   
& $\pm      0$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)\rangle $} & \multicolumn{1}{ |c|}{  0.193} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $+   148$   
& ${}_{-     86}^{+     89} $
& ${}_{-    130}^{+    130} $
& $\pm     41$   
& $\pm     60$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $+    85$   
& ${}_{-     91}^{+     81} $
& ${}_{-    130}^{+    130} $
& $\pm     49$   
& $\pm     59$   
\\ \cline{3-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    437}^{+    696} $
& ${}_{-     95}^{+     95} $
& $\pm     85$   
& $\pm      0$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{  0.286} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $   -105$   
& ${}_{-    369}^{+    552} $
& ${}_{-     95}^{+     95} $
& $\pm     78$   
& $\pm     72$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $   -558$   
& ${}_{-    364}^{+    548} $
& ${}_{-     95}^{+     95} $
& $\pm     95$   
& $\pm     71$   
\\ \cline{3-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    359}^{+    248} $
& ${}_{-    395}^{+    395} $
& $\pm     57$   
& $\pm      0$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{$\langle m(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{  0.331} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $+   113$   
& ${}_{-    261}^{+    253} $
& ${}_{-    395}^{+    395} $
& $\pm     33$   
& $\pm    120$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $+   515$   
& ${}_{-    271}^{+    248} $
& ${}_{-    395}^{+    395} $
& $\pm     68$   
& $\pm    118$   
\\ \cline{3-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    386}^{+    345} $
& ${}_{-   1068}^{+   1068} $
& $\pm    540$   
& $\pm      0$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{$\langle E(\ell^+\ell^-)\rangle $} & \multicolumn{1}{ |c|}{  0.556} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $+   180$   
& ${}_{-    451}^{+    468} $
& ${}_{-   1068}^{+   1068} $
& $\pm    474$   
& $\pm    196$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $+     6$   
& ${}_{-    407}^{+    415} $
& ${}_{-   1068}^{+   1068} $
& $\pm    559$   
& $\pm    194$   
\\ \cline{3-8}
\cline{1-8}
 \\[-1.25em]
\cline{1-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\bbfourl $\phantom{\Big|}$}
& $+     0$   
& ${}_{-    186}^{+    167} $
& ${}_{-    259}^{+    259} $
& $\pm     93$   
& $\pm      0$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{$\langle \pT(\ell^+)+\pT(\ell^-)\rangle $} & \multicolumn{1}{ |c|}{  0.389} & \multicolumn{1}{ |c|}{\ttbnlodec $\phantom{\Big|}$}
& $+   275$   
& ${}_{-    166}^{+    170} $
& ${}_{-    259}^{+    259} $
& $\pm     72$   
& $\pm    114$   
\\ \cline{3-8}
\multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{} & \multicolumn{1}{ |c|}{\hvq $\phantom{\Big|}$ }
& $+   104$   
& ${}_{-    178}^{+    164} $
& ${}_{-    259}^{+    259} $
& $\pm    101$   
& $\pm    113$   
\\ \cline{3-8}
\cline{1-8}
\end{tabular}

